Quadratically Enriched Tropical Intersections

Using tropical geometry one can translate problems in enumerative geometry to combinatorial problems. Thus tropical geometry is a powerful tool in enumerative geometry over the complex and real numbers. Results from $\mathbb{A}^1$-homotopy theory allow to enrich classical enumerative geometry questions and get answers over an arbitrary field. In the resulting area, $\mathbb{A}^1$-enumerative geometry, the answer to these questions lives in the Grothendieck-Witt ring of the base field $k$. In this paper, we use tropical methods in this enriched set up by showing B\'ezout's theorem and a generalization, namely the Bernstein-Kushnirenko theorem, for tropical hypersurfaces enriched in $\operatorname{GW}(k)$.

==> 4etic.tex <==
% !TeX root=main.tex

\section{Enriched tropical intersection multiplicity for curves}
\label{section:curves}
For expository reasons, we first prove our main theorem for tropical curves and do the general case in section \ref{section:Higher dimensions}.
Throughout this section we will consider tropical curves enriched over a perfect field $k$ of characteristic not equal to $2$. However, our computations hold as long as the fields of definition of the intersection points are separable extensions of $k$. %and hence, the trace form the \'etale algebras defined by these extensions can be computed.

Let $\tC_1$ and $\tC_2$ be two enriched tropical curves with enriched Viro polynomials
\[f_1=\sum_{I\in A} \alpha_Ix^{i_1}y^{i_2}t^{\phi(I)}
\text{ and } 
f_2=\sum_{J\in B} \beta_Ix^{j_1}y^{j_2}t^{\psi(J)},\] 
respectively, where both sums are over some finite subsets $A,B$ of $\Z^2$ and $\phi\colon A\longrightarrow \Z$ and $\psi\colon B\longrightarrow \Z$ are convex functions.


\begin{df}
We define the \emph{enriched intersection multiplicity} of $\tC_1$ and $\tC_2$ at $p\in\tC_1\cap\tC_2$ to be
\[\mult_p(\tC_1,\tC_2)\coloneqq \Tr_{E_t/k\Puiseux}
\qinv{\det \operatorname{Jac}(f_1,f_2)(z)}\in \GW(k\Puiseux)\]
where $z$ is a solution to $f_1=f_2=0$ with $-\operatorname{val}(z)=p$ and $E_t$ is the coordinate ring of all such $z$. %which we assume to be \'etale over $k\Puiseux$.
\end{df}
\begin{rmk} With the notation above, let $d_1=\deg f_1$ and $d_2=\deg f_2$ (in $x$ and $y$, not in $t$) and
note that our definition of the enriched intersection multiplicity $\mult_p(\tC_1,\tC_2)$ equals the local index (see Definition \ref{df:local index}) of the section defined by $(f_1,f_2)$ of $\mathcal{O}_{\mathbb{P}^2 _{k\Puiseux}}(d_1)\oplus \mathcal{O}_{\mathbb{P}^2 _{k\Puiseux}}(d_2)$ at the zeros that tropicalize to $p$.
\end{rmk}

%\subsection{Quadratically invariant intersection}

Assume that $\tC_1$ and $\tC_2$ intersect tropically transversally at $p$ and assume $z\in \bar{k}\Puiseux^2$ tropicalizes to $p$.
Then the maximum of $-\operatorname{val}(f_1(z))$ and $-\operatorname{val}(f_2)(z)$ is attained exactly twice.
This implies that the initial $z_\circ=(z_1,z_2)$ of $z$ has to satisfy \emph{binomial equations} (by a binomial we mean a polynomial with two summands) 
\[f_1'=\alpha_Iz_1^{i_1}z_2^{i_2}+\alpha_{I'}z_1^{i_1'}z_2^{i_2'}=0\]
and
\[f_2'=\beta_Jz_1^{j_1}z_2^{j_2}+\beta_{J'}z_1^{j_1'}z_2^{j_2'}=0.\]
These are exactly the summands of $f_1(x,y)$ and $f_2(x,y)$ for which the maximum of $-\operatorname{val}$ is attained.
We call 
\[f_1'=\alpha_Ix^{i_1}y^{i_2}+\alpha_{I'}x^{i_1'}y^{i_2'}=0\]
and
\[f_2'=\beta_Jx^{j_1}y^{j_2}+\beta_{J'}x^{j_1'}y^{j_2'}=0.\]
\emph{local binomial equations} at $p$.
In particular, we get that
the coordinate ring of the initials of the points that tropicalize to $p$ equals
\[E\coloneqq\frac{k[x^{\pm1},y^{\pm1}]}{(f_1',f_2')}\]
where $f_1',f_2'\in k[x,y]$ are the {local binomial equations} at $p$.

Recall from Example \ref{ex:GW of Puiseux} that $\GW(k)\cong \GW(k\Puiseux)$. The next theorem identifies the enriched intersection multiplicity $\mult_p(\tC_1,\tC_2)\in \GW(k\Puiseux)$ with an element of $\GW(k)$ via this isomorphism.
\begin{thm}
\label{thm:enriched intersection multiplicity}
Let $\tC_1$ and $\tC_2$ be enriched tropical curves in $\R^2$ with Newton polygons $\Delta_1$ and~$\Delta_2$, respectively.
If $\tC_1$ and $\tC_2$ intersect transversely at $p=(p_1,p_2)\in\mathbb{R}^2$, then the enriched intersection multiplicity~$\mult_p(\tC_1,\tC_2)$ at $p$ is given by
\[
\Tra[E/k]{
\qinv{ 
\det \left(\Delta I,\Delta J \right)\alpha_{I}\beta_{J} z_{\circ}^{I+J-e_{1}-e_2} }}\in \GW(k)
\] 
where $\Tr$ is the trace map, $E$ the coordinate ring of all $z_\circ$ which are initials of solutions ${z\in \bar{k}\Puiseux^2}$ with $-\operatorname{val}(z)=p$, 
$f_1'=\alpha_Ix^{i_1}y^{i_2}+\alpha_{I'}x^{i_1'}y^{i_2'}$ and $f_2'=\beta_Jx^{j_1}y^{j_2}+\beta_{J'}x^{j_1'}y^{j_2'}$ are the local binomial equation of $\tC_1$ at $p$ and of $\tC_2$ at~$p$, respectively, and
$\Delta I=I-I'$, $\Delta J=J-J'$. 
\end{thm}

\begin{rmk}
In particular, we see that if the two enriched tropical curves $\tC_1$ and $\tC_2$ intersect tropically transversally at $p$, then $\det \operatorname{Jac}(\tp)\neq 0$ and we can use \eqref{eq:nonrational}. 
%Hence, the two curves in $\mathbb{A}^2_{k\Puiseux}$ intersect transversally at $\tp$.
\end{rmk}


\begin{proof}
%For an algebraically closed field, the quadratic multiplicity at a intersection point of two curves $\tC_1$ and $\tC_2$ is given by the class of the bilinear form associated to the evaluation of the Jacobian of the equations defining the curves at the intersection point. In the general case, it is given by the image by the trace map over a separable field extension defining a solution, of the class of the bilinear evaluation of the Jacobian of the equations defining the curves at the intersection point. We detail the trace map in Section~\ref{ss:trace}. 


In order to compute the evaluation of the determinant of the Jacobian, let us remark that we have an isomorphism between the Grothendieck-Witt ring of the field of Puiseux series over~$k$ and the Grothendieck-Witt ring of the field~$k$ given by the initial map
\[ \Ini\colon
\begin{array}{ccc}
\GW\left(k\Puiseux\right) &   \lra   &  \GWk\\
f(t)            &   \lmt   &    \Ini(f)
\end{array}.
\]
Hence, it suffices to compute the initial of the to the evaluation of the Jacobian of the equations defining the curves at the intersection point. 
Let $\tp(t)\in\bar{k}\Puiseux^2$ such that 
\[
\sum_{K\in \Delta_1\cap\Lambda}\alpha_K \tp^{K}t^{\phi(K)}=
\sum_{K\in \Delta_2\cap\Lambda}\beta_K \tp^{K}t^{\varphi(K)}=0,
\]
and such that $-val(\tp)=p$ and let $\zn=\Ini(\tp)$ be the initial of the lifting $\tp$.

Since $\alpha_{I} z^{I}t^{\phi(I)}+\alpha_{I'} z^{I'}t^{\phi(I')}$ is the local equation of $\tC_1$ at $p$, and
$\beta_{J} z^{J}t^{\varphi(J)}+\beta_{J'} z^{J'}t^{\varphi(J')}$ is the local equation of $\tC_2$ at~$p$, the Jacobian of the intersection at $\tp$ is given by the determinant
\begin{equation}\label{eq:Jacob}
\begin{vmatrix}
i_1\alpha_I z^{I-e_1}t^{\phi(I)}+i_1' \alpha_{I'} z^{I'-e_1}t^{\phi(I')} &
i_2\alpha_I z^{I-e_2}t^{\phi(I)}+i_2' \alpha_{I'} z^{I'-e_2}t^{\phi(I')} \\
j_1\beta_J z^{J-e_1}t^{\varphi(J)}+j_1'\beta_{J'} z^{J'-e_1}t^{\varphi(J')} &
j_2\beta_J z^{J-e_2}t^{\varphi(J)}+j_2'\beta_{J'} z^{J'-e_2}t^{\varphi(J')}
\end{vmatrix},
\end{equation}
evaluated at $\tp$. To compute its initial we should first compute its valuation.
We have that~$\tp$ satisfies 
\begin{equation}\label{eq:init}
\alpha_I\tp^{I}t^{\phi(I)}+\alpha_{I'} \tp^{I'}t^{\phi(I')}=0,\quad \beta_J \tp^{J}t^{\varphi(J)}+\beta_{J'} \tp^{J'}t^{\varphi(J')}=0.
\end{equation}
Then, we have that $\Val{\alpha_I\tp^{I}t^{\phi(I)}}=\Val{\alpha_{I'} \tp^{I'}t^{\phi(I')}}$, 
and~$\Val{\beta_J\tp^{J}t^{\varphi(J)}}=\Val{\beta_{J'} \tp^{J'}t^{\phi(J')}}$.
Equivalently,
\[-p_1i_1-p_2i_2+\phi(I)=-p_1i_1'-p_2i_2'+\phi(I'), \text{ and }
 -p_1j_1-p_2j_2+\varphi(J)=-p_1j_1'-p_2j_2'+\phi(J'),\]
where $I=(i_1,i_2)$, $I=(i_1',i_2')$, $J=(J_1,J_2)$, and $J'=(J_1',J_2')$. This implies
\[\val(i_1\alpha_I \tp^{I-e_1}t^{\phi(I)})=
-p_1(i_1-1)-p_2i_2+\phi(I)=-p_1(i_1'-1)-p_2i_2'+\phi(I')
=\val(i_1' \alpha_{I'} \tp^{I'-e_1}t^{\phi(I')}),\]
\[\val(i_2\alpha_I \tp^{I-e_2}t^{\phi(I)})=
-p_1i_1-p_2(i_2-1)+\phi(I)=-p_1i_1'-p_2(i_2'-1)+\phi(I')
=\val(i_2' \alpha_{I'} \tp^{I'-e_2}t^{\phi(I')}),\]
\[\val(j_1\beta_J \tp^{J-e_1}t^{\varphi(J)})=
-p_1(j_1-1)-p_2j_2+\varphi(J)=-p_1(j_1'-1)-p_2j_2'+\varphi(J')
=\val(j_1' \beta_{J'} \tp^{J'-e_1}t^{\varphi(J')}),\]\[\val(j_2\beta_J \tp^{J-e_2}t^{\varphi(J)})=
-p_1j_1-p_2(j_2-1)+\varphi(J)=-p_1j_1'-p_2(j_2'-1)+\varphi(J')
=\val(j_2' \beta_{J'} \tp^{J'-e_2}t^{\varphi(J')}).\]

Let us remark that, since the valuation of the product is the sum of the valuation of the factors, the valuation of the product of the entries in the diagonal is equal to the valuation of the product of the entries in the antidiagonal.
Hence, the valuation of the determinant of the Jacobian~\eqref{eq:Jacob} equals $-p_1(i_1-1)-p_2i_2+\phi(I)+-p_1j_1-p_2(j_2-1)+\varphi(J)$ given that the corresponding term does not vanish. 

Let us start by computing the terms of every entry of degree corresponding to the calculated valuations. 
Using~\eqref{eq:init} the sum $i_1\alpha_I z^{I-e_1}t^{\phi(I)}+i_1' \alpha_{I'-e_1} z^{I'}t^{\phi(I')}$ evaluated at $\tp$ equals
\begin{align*}
i_1\alpha_I \tp^{I-e_1}t^{\phi(I)}+i_1' \alpha_{I'} \tp^{I'-e_1}t^{\phi(I')}
&= i_1\alpha_I \tp^{I-e_1}t^{\phi(I)}+i_1'\tp^{-e_1}
\left(\alpha_{I'} \tp^{I'}t^{\phi(I')}\right)\\
&= i_1\alpha_I \tp^{I-e_1}t^{\phi(I)}+i_1'\tp^{-e_1}
\left(-\alpha_{I} \tp^{I}t^{\phi(I)}\right)\\
&= \left( i_1- i_1'\right)
\left(\alpha_{I} \tp^{I-e_1}t^{\phi(I)}\right),\\
\end{align*}
whose term of degree~$\val(i_1\alpha_I \tp^{I-e_1}t^{\phi(I)})$ is $\left( i_1- i_1'\right)\left(\alpha_{I} \zn^{I-e_1}\right)$.
Similarly, the term of degree
$\val(i_2\alpha_I \tp^{I-e_2}t^{\phi(I)})$ of the sum $i_2\alpha_I z^{I-e_2}t^{\phi(I)}+i_2' \alpha_{I'} z^{I'-e_2}t^{\phi(I')}$ is 
$\left( i_2- i_2'\right)\left(\alpha_{I} \zn^{I-e_2}\right)$;
the term of degree $\val(j_1\beta_J \tp^{J-e_1}t^{\varphi(J)})$ of the sum 
$j_1\beta_J z^{J-e_1}t^{\varphi(J)}+j_1'\beta_{J'} z^{J'-e_1}t^{\varphi(J')}$ is 
$\left( j_1- j_1'\right)\left(\beta_{J} \zn^{J-e_1}\right)$; and lastly, the term of degree $\val(j_2\beta_J \tp^{J-e_2}t^{\varphi(J)})$ of the sum
$j_2\beta_J z^{J-e_2}t^{\varphi(J)}+j_2'\beta_{J'} z^{J'-e_2}t^{\varphi(J')}$ is~
$\left( j_2- j_2'\right)\left(\beta_{J} \zn^{J-e_2}\right)$.
Therefore, the initial of the determinant of the Jacobian~\eqref{eq:Jacob} is
\[
\left[\left( i_1- i_1'\right)\left( j_2- j_2'\right)-\left( i_2- i_2'\right)\left( j_1- j_1'\right)
\right]
\left(\alpha_{I}\beta_{J} \zn^{I+J-e_1-e_2}\right),
\]
which is non-zero since $\alpha_I, \beta_J, \zn\in k^*$, and the curves $C_1$ and $C_2$ intersect tropically transversally.
\end{proof}




\begin{lm}
\label{lm: symmetry}
If we exchange the roles of $I$ and $I'$, or those of $J$ and $J'$, the product
\[\det \left( \Delta I,\Delta J\right)\alpha_{I}\beta_{J} z_{\circ}^{I+J-e_{1}-e_2}\]
is invariant.
\end{lm}
\begin{proof}
This follows directly from equation~\eqref{eq:init}. Indeed, the initial $\zn$ satisfies $\alpha_I\zn^{I}+\alpha_{I'}\zn^{I'}=0$. Hence, if we exchange the roles of $I$ and $I'$ we have
\begin{align*}
\det((I'-I),\Delta J)\alpha_{I'}\beta_{J} z_{\circ}^{I'+J-e_{1}-e_2}
&=\det((I'-I),\Delta J) 
\left(\alpha_{I'}\zn^{I'}\right)\beta_{J} z_{\circ}^{J-e_{1}-e_2}\\
&=\det((I'-I),\Delta J) 
\left(-\alpha_{I}\zn^{I}\right)\beta_{J} z_{\circ}^{J-e_{1}-e_2}\\
&=\det((I-I'),\Delta J)\alpha_{I}\beta_{J} z_{\circ}^{I+J-e_{1}-e_2}.\\
\end{align*}
The same argument proves the invariance with respect to the exchange of $J$ and $J'$.
\end{proof}

\subsection{A combinatorial formula for $\mult_p(\tC_1,\tC_2)$}


Recall that the intersections of two tropical curves $C_1$ and $C_2$ correspond to parallelograms in the dual subdivision of $C_1\cup C_2$ and that the classical tropical intersection multiplicity at an intersection point equals the area of this parallelogram, that means the interesection multiplicity can be read of the dual subdivision $\operatorname{DS}(C_1\cup C_2)$ of $C_1\cup C_2$. Our goal is to find a way to determine the enriched intersection multiplicity with the help of the dual subdivision of two enriched tropical curves $\tC_1$ and $\tC_2$.


Each tropically transverse intersection point $p$ of $\tC_1$ and $\tC_2$ lies on an edge of $C_1$, respectively~$C_2$, which separates two connected components of $\R^2\setminus C_1$, respectively of $\R^2\setminus C_2$. Each of these connected components has a coefficient assigned. Let us call these coefficients $\alpha_I$ and~$\alpha_{I'}$, respectively $\beta_J$ and $\beta_{J'}$, as in Figure \ref{fig:coeffprod}. Recall from Lemma \ref{lm:coefficient curves} that the coefficients of the components of $\tC_1\cup \tC_2$ adjacent to intersection point $p$ are $\alpha_I\beta_J$, $\alpha_{I'}\beta_J$, $\alpha_I\beta_{J'}$ and $\alpha_{I'}\beta_{J'}$ as in figure~\ref{fig:coeffprod}.
In particular, the vertices $I+J$, $I'+J$, $I+J'$ and $I'+J'$ of the parallelogram dual to $p$ in the dual subdivision of $\tC_1\cup \tC_2$ have coefficients $\alpha_I\beta_J$, $\alpha_{I'}\beta_J$, $\alpha_I\beta_{J'}$ and $\alpha_{I'}\beta_{J'}$, respectively.

Let $v$ be a corner vertex of a parallelogram $P$ in $\operatorname{DS}(\tC_1\cup \tC_2)$ dual to a point $p\in \tC_1\cap \tC_2$. Set

\begin{equation}
\label{eq:sign}
\epsilon_P(v)\coloneqq\begin{cases}
+1 & \text{first $C_1$ then $C_2$} \\
-1 & \text{first $C_2$ then $C_1$}
\end{cases}\end{equation}
when walking around the vertex inside the parallelogram anticlockwise (see Figure \ref{fig:sign}) and note that this equals the sign of $\det(\pm\Delta I,\pm\Delta J)$, where each $\Delta I,\Delta J$ is oriented in a way that the vertices $v\pm\Delta I,v\pm\Delta J\in P$.

\begin{figure}[t]
\begin{tabular}{ccc}
\includegraphics{Figures/sign0.pdf}&
\includegraphics{Figures/sign1.pdf}&
\includegraphics{Figures/sign2.pdf}
\end{tabular}
\caption{The dual parallelogram associated to an intersection point and a local picture of signed vertices.\label{fig:sign}}
\end{figure}

%\begin{lm}
%The absolute value of $\triangle I\cdot\triangle J^{\bot}$ is equal to the classical intersection multiplicity of $C_1$ and $C_2$ at $p$
%\[\vert \triangle I\cdot\triangle J^{\bot}\vert=\operatorname{mult}_p(C_1,C_2).\]
%Furthermore, it holds for the sign $\epsilon$ of the intersection that
%\[\epsilon=\operatorname{sign}(\Delta I\cdot\Delta J^{\bot}).\]
%\end{lm}
%\begin{proof}
%Let us remark that
%\[\triangle I\cdot\triangle J^{\bot}=\det\left(\triangle I,\triangle J\right)\]
%The first statement follows from the characterization of the classical tropical multiplicity as the area of the paralellogram in the dual subdivision associated to the point.
%The second statement follows from the fact that the determinant $\det(u,v)$ equals the area of the paralellogram spanned by $u$ and $v$ if and only if the ordered couple $(u,v)$ have an anti-clockwise orientation.
%\end{proof}

\begin{rmk}
\label{rmk:signs}
Note that the sign of the vertex $I+J$ is the same as the sign of $I'+J'$ and opposite of the sign of $I'+J$ and $I+J'$.
\end{rmk}

%\begin{df}
%Then the \emph{enriched intersection multiplicity} of $\widetilde{C}_1$ and $\widetilde{C}_2$ at $p$ is
%\begin{equation}
%\label{eq:def mult}
%\widetilde{\operatorname{mult}}_p(\widetilde{C}_1,\widetilde{C}_2)=\sum_{l=1}^{q}\qinv{\epsilon^{(q)}\alpha_I\beta_J}+\frac{m-q}{2}\cdot h \in \GW(k).    
%\end{equation}
%\end{df}

%\begin{thm}
%\label{thm:intersection mult dual subdivision}
%For an intersection point $p$ of two enriched tropical curves $\widetilde{C}_1$ and $\widetilde{C}_2$ with $\operatorname{mult}_p(C_1,C_2)=1$ (classical intersection multiplicity), the enriched intersection multiplicity $\widetilde{\operatorname{mult}}_p(\widetilde{C}_1,\widetilde{C}_2)$ coincides with the calculation in Theorem \ref{thm:enriched intersection multiplicity}, that is,
%it holds that 
%\[\widetilde{\operatorname{mult}}_p(C_1,C_2)=\Tr_{E/k}\qinv{\left(\triangle I \cdot {\triangle J}^{\bot} \right)\alpha_{I}\beta_{J} z_{\circ}^{I+J-e_{1}-e_2}}\in \GW(k)\]
%where $E=\frac{k[x,y]}{(\alpha_Iz_\circ^I+\alpha_{I'}z_\circ^{I'},\beta_Jz_\circ^J+\beta_{J'}z_\circ^{J'})}$.
%\end{thm}

We are now ready to state our main theorem for in the case of curves.
Recall that we say that a vertex $v\in \Z^2$ is \emph{odd} if $v\equiv(1,1)$ in $(\Z/2\Z)^2$.

\begin{thm}
\label{thm:mainthmcurves}
Let $q$ be the number of odd corner vertices of the parallelogram $P$ dual to $p$ in the dual subdivision of $\tC_1\cup \tC_2$.
Let $m$ be the classical intersection multiplicity at $p$ given by the area of the parallelogram $P$. % $m=\operatorname{mult}_p(C_1,C_2)=\operatorname{Area}(P)$.
Then,
\[\mult_p(\tC_1,\tC_2)=\sum_{v\text{ odd}}\qinv{ \epsilon_P(v)\alpha_v} +\frac{m-q}{2}\;h\in \GW(k)\]
where the sum runs over all odd corners of $P$ and $\alpha_v=\alpha_I\beta_J$ is the coefficient of $v=I+J$.
\end{thm}

\begin{ex}
\label{ex:enrichedMult}
Figure \ref{fig:innerdual} shows the dual subdivision of the union of the tropical cubic and tropical conic in Figure \ref{fig:intcurves}. The parallelograms corresponding to the intersections are highlighted. Let~$\alpha_{(3,1)}$ and $\alpha_{(1,3)}$ be the coefficients of the two odd vertices $(3,1)$ and $(1,3)$ of the dual subdivision. Then the intersection corresponding to the upper left parallelogram has enriched intersection multiplicity $\qinv{\alpha_{(1,3)}}$, the one corresponding to the upper right parallelogram has enriched intersection multiplicity $\qinv{ -\alpha_{(1,3)}} +\qinv{-\alpha_{(3,1)}}$ and the last one has enriched intersection multiplicity $h+\qinv{\alpha_{(3,1)}}$.

\begin{figure}[t]
    \centering
    \includegraphics{Figures/TropIntDual000.pdf}
    \caption{Odd vertices and their adjacent parallelograms in the dual subdivision of the curves in Figure~\ref{fig:intcurves}.}
    \label{fig:innerdual}
\end{figure}
\end{ex}



\subsection{Proof of Theorem \ref{thm:mainthmcurves}}





Recall that
\[E=\frac{k[x^{\pm1},y^{\pm 1}]}{(f_1',f_2')}\]
with $f_1'=\alpha_Ix^{i_1}y^{i_2}+\alpha_{I'}x^{i_1'}y^{i_2'}$ and $f_2'=\beta_Jx^{j_1}y^{j_2}+\beta_{J'}x^{j_1'}y^{j_2'}$ the local binomial equations at $p$,
%and assume that $E$ is finite \'{e}tale over $k$.
is the coordinate ring of the initials of points that tropicalize to $p$.
In Theorem \ref{thm:enriched intersection multiplicity}
we computed the enriched intersection multiplicity of $\tC_1$ and $\tC_2$ at $p$ to be 
\[\Tr_{E/k}\qinv{\det \left(\Delta I, \Delta J\right) \alpha_{I}\beta_{J} z_{\circ}^{I+J-e_{1}-e_2}}\in \GW(k).\]


We use the notation
\[\Delta i_1= i_1-i_1'\text{, }\Delta i_2=i_2-i_2'\text{, }\Delta j_1=j_1-j_1'\text{, }\Delta j_2=j_2-j_2'.\]


In order to use our formulas for the trace in Proposition \ref{prop:traces}, we first show that $E$ is of the following form.
\begin{prop}
\label{prop:Ecurves}
Let $m=\operatorname{mult}_p(C_1,C_2)$ be the classical intersection multiplicity of $C_1$ and $C_2$ at $p$.
Then there is $d\in \Z_{\ge1}$ such that $d$ divides $m$, and there are $D_1\in k$ and $D_2\in L\coloneqq\frac{k[w]}{(w^{\frac{m}{d}}-D_1)}$ such that $E=\frac{L[w]}{(w^d-D_2)}$.
\end{prop}


\begin{proof}

We aim to solve for $x$ and $y$ given the two equations 
\begin{equation}
\label{eq:alpha}
    \alpha_Ix^{i_1}y^{i_2}+\alpha_{I'}x^{i_1'}y^{i_2'}=0 \Leftrightarrow -\frac{\alpha_{I}}{\alpha_{I'}}=x^{\Delta i_1}y^{\Delta i_2}
\end{equation}
and 
\begin{equation}
\label{eq:beta}
    \beta_Jx^{j_1}y^{j_2}+\beta_{J'}x^{j_1'}y^{j_2'}=0\Leftrightarrow -\frac{\beta_{J}}{\beta_{J'}}=x^{\Delta j_1}y^{\Delta j_2}.
\end{equation}

We know that $\det \left(\Delta I,\Delta J\right)=\Delta i_1\Delta j_2-\Delta i_2\Delta j_1=\pm m$.

Let $d=\operatorname{gcd}(\Delta i_1,\Delta j_1)$.
Then $\eqref{eq:alpha}^{-\frac{\Delta j_1}{d}}\cdot \eqref{eq:beta}^{\frac{\Delta i_1}{d}}$ yields
\[
    y^{\frac{m}{d}}=\left(-\frac{\alpha_{I'}}{\alpha_{I}}\right)^{\frac{\Delta j_1}{d}}\cdot \left(-\frac{\beta_{J}}{\beta_{J'}}\right)^{\frac{\Delta i_1}{d}}\eqqcolon D_1.
\]
So $y\in L=\frac{k[w]}{(w^{\frac{m}{d}}-D_1)}$.
Since $\operatorname{gcd}(\frac{\Delta i_1}{d},\frac{\Delta j_1}{d})=1$
, there are $r,s\in \Z$ such that 
\[
    r\cdot \frac{\Delta i_1}{d}+s\cdot \frac{\Delta j_1}{d}=1.
\]


Now $\eqref{eq:alpha}^{r}\cdot \eqref{eq:beta}^s$ yields 
\[
    x^d=y^{-\Delta i_2\cdot r-\Delta j_2 \cdot s}\cdot \left(-\frac{\alpha_{I'}}{\alpha_I}\right)^r\cdot \left(-\frac{\beta_{J'}}{\beta_J}\right)^s\eqqcolon D_2
\]
and thus $x\in \frac{L[w]}{(w^d-D_2)}$.

\end{proof}

It follows that 
\[\Tr_{E/k}\qqinv{ \det(\Delta I, \Delta J )\alpha_{I}\beta_{J} z_{\circ}^{I+J-e_{1}-e_2}}=\Tr_{L/k}\circ \Tr_{E/L}\qqinv{ \det(\Delta I, \Delta J )\alpha_{I}\beta_{J} z_{\circ}^{I+J-e_{1}-e_2}},\]
which we can compute with the help of Proposition \ref{prop:traces}.

\begin{lm}
\label{lm:m odd}The classical intersection multiplicity
$m=\operatorname{mult}_p(C_1,C_2)$ is odd if and only if the parallelogram $P$ dual to $p$ has exactly one odd vertex.
\end{lm}
\begin{proof}
We first show that if $m$ is odd, then all four vertices of $P$ are pairwise different in ${(\Z/2\Z)^2}$, and thus there is exactly one odd vertex.
We know that $\Delta I\cdot \Delta J^{\bot}=\Delta i_1 \cdot \Delta j_2-\Delta i_2\cdot \Delta j_1$ is odd.
So one of the summands must be odd and the other even. Without loss of generality we can assume that both $\Delta i_1$ and $\Delta j_2$ are odd. Then at least one out of $\Delta i_2$ and $\Delta j_1$ is even. So there are three cases we need to check. In all the cases 
\begin{equation}
\label{eq:4 vertices}
\begin{pmatrix}0\\0\end{pmatrix}, \begin{pmatrix}\Delta i_1\\ \Delta i_2\end{pmatrix}, \begin{pmatrix}\Delta j_1\\ \Delta j_2\end{pmatrix},\begin{pmatrix}\Delta i_1+\Delta j_1\\ \Delta i_2+\Delta j_2\end{pmatrix}\end{equation}
are pairwise different in $(\Z/2\Z)^2$. It follows that 
\[I+J, I+J+\Delta I=I'+J, I+J+\Delta J=I+J', I+J+\Delta I+\Delta J=I'+J'\]
are pairwise different. 

Now assume that there is exactly one odd vertex. This implies that the four vectors in \eqref{eq:4 vertices} are pairwise different in $\Z/2\Z\times \Z/2\Z$. 
The area of this parallelogram is a non-zero element in $\Z/2\Z$, hence it is odd. 
\end{proof}


\begin{proof}[Proof of Theorem \ref{thm:mainthmcurves}]
\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \begin{tikzpicture}[scale=0.7]
\draw[red,very thick] (-3,-2)--(3,2);
\draw[blue,very thick] (0,-3)--(0,3);
\filldraw[black] (0,0) circle (2pt) node[anchor=east]{$p$};
\node at (-1,1.5) {$\alpha_I\beta_{J'}$};
\node at (1,2) {$\alpha_{I'}\beta_{J'}$};
\node at (-1,-2) {$\alpha_I\beta_J$};
\node at (1,-1.5) {$\alpha_{I'}\beta_J$};
\end{tikzpicture}
\caption{Intersection at $p$}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \begin{tikzpicture}
\fill[gray!10!white,thick] (-2,0)--(0,0)--(2,-3)--(0,-3)--cycle;
\draw[blue,thick] (-2,0)--(0,0);
\draw[blue,thick] (2,-3)--(0,-3);
\draw[red,thick] (0,0)--(2,-3);
\draw[red,thick] (0,-3)--(-2,0);
\node at (0,-1.5) {$P$};
\node at (0.5,0.2) {$I'+J'$};
\node at (-2.4,0.2) {$I+J'$};
\node at (-0.4,-3.2) {$I+J$};
\node at (2.5,-3.2) {$I'+J$};
\node[blue] at (1,-3.3) {$\Delta I$};
\node[red] at (-1.5,-1.5) {$\Delta J$};
\end{tikzpicture} 
\caption{Dual parallelogram $P$}
     \end{subfigure}
        \caption{An enriched tropical intersection together with the dual parallelogram.}
         \label{figure:EnrichedIntersection}
\end{figure}

Recall from the proof of Proposition \ref{prop:Ecurves} that
\begin{equation}
\label{eq:D1}
   D_1=\left(-\frac{\alpha_{I'}}{\alpha_{I}}\right)^{\frac{\Delta j_1}{d}}\cdot \left(-\frac{\beta_{J}}{\beta_{J'}}\right)^{\frac{\Delta i_1}{d}}
\end{equation}
and
\begin{equation}
\label{eq:D2}
    D_2= z_2^{-\Delta i_2\cdot r-\Delta j_2 \cdot s}\cdot \left(-\frac{\alpha_{I}}{\alpha_{I'}}\right)^r\cdot \left(-\frac{\beta_{J}}{\beta_{J'}}\right)^s,
\end{equation}
where $r$ and $s$ are integers such that 
\begin{equation}
\label{eq:ra+ba=1}
    r\cdot\frac{\Delta i_1}{d}+s\cdot \frac{\Delta j_1}{d}=1.
\end{equation}
Furthermore, we set
\begin{equation}
\label{eq:D2'}
    D_2'\coloneqq \left(-\frac{\alpha_{I}}{\alpha_{I'}}\right)^r\cdot \left(-\frac{\beta_{J}}{\beta_{J'}}\right)^s.
\end{equation}
Recall that 
\begin{equation}
\label{eq:m}
    m=\vert \Delta i_1\cdot \Delta j_2-\Delta i_2\cdot \Delta j_1\vert
\end{equation}
equals the classical intersection multiplicity of $C_1$ and $C_2$ at $p$, and that 
\begin{equation}
\label{eq:gcd}
d=\gcd(\Delta i_1,\Delta j_1).
\end{equation}
Let $\epsilon\coloneqq\epsilon_P(I+J)$ be the sign of the vertex $I+J$ of $P$ and write $z_\circ=(z_1,z_2)\in \bar{k}^2$.

We prove the Theorem step by step going through all possible cases.
We already know that the rank of the resulting form is $m=\operatorname{dim}_kE$. So we can compute everything in $\W(k)$, and then add hyperbolic summands to get an element of $\GW(k)$ of the correct rank. 

\textbf{$P$ has no odd vertex}: First observe that $P$ has an odd vertex if $m$ is odd by Lemma \ref{lm:m odd}, so we know that $m$ is even in this case. 

\begin{enumerate}
\item
If $d$ is odd, then at least one out of $\Delta i_1$ and $\Delta j_1$ must be odd and we can choose $I$ and $J$ such that $i_1+j_1-1$ is even by Lemma \ref{lm: symmetry}. In this case $i_2+j_2-1$ is odd otherwise there would be an odd vertex.
Then 
\begin{align*}
\Tr_{E/L}\qqinv{ \epsilon m \alpha_I\beta_Jz_\circ^{I+J-e_1-e_2}})&=\Tr_{E/L}\qqinv{ \epsilon m \alpha_I\beta_Jz_1^{i_1+j_1-1}z_2^{i_2+j_2-1}}\\&
=\Tr_{E/L}\qqinv{ \epsilon m \alpha_I\beta_Jz_2}\\
&=\qinv{ \epsilon m d \alpha_I\beta_Jz_2}
\end{align*}
in $\operatorname{W}(L)$. Taking $\Tr_{L/k}$ we get $0\in \operatorname{W}(k)$ by Proposition \ref{prop:traces} since $z_2\not\in k$ and $\frac{m}{d}$ must be even because $m$ is even.
\item
If $d$ is even, then $\Delta i_1$ and $\Delta j_1$ are both even. So $i_1+j_1-1, i_1'+j_1-1, i_1+j_1'-1,i_1'+j_1'-1$ are either all even or all odd. 
If they are all odd, then 
\[\Tr_{E/L}\qqinv{ \epsilon m \alpha_I\beta_Jz_\circ^{I+J-e_1-e_2}}=\Tr_{E/L}\qqinv{ \epsilon m \alpha_I\beta_Jz_2^{i_2+j_2-1}z_1}=0\]
in $\operatorname{W}(L)$ for any choice of $I$ and $J$ by Proposition \ref{prop:traces}
and our statement holds.
\item
If $i_1+j_1-1, i_1'+j_1-1, i_1+j_1'-1,i_1'+j_1'-1$ are all even, then $i_2+j_2-1, {i_2'+j_2-1}, {i_2+j_2'-1},$ ${i_2'+j_2-1}$ must all be odd, otherwise there would be an odd vertex. This implies that $\Delta i_2$ and $\Delta j_2$ are both even and hence, both $d$ and $\frac{m}{d}$ are even. Thus
\[\Tr_{E/L}\qqinv{ \epsilon m \alpha_I\beta_Jz_\circ^{I+J-e_1-e_2}}=\Tr_{E/L}\qqinv{ \epsilon m \alpha_I\beta_Jz_2}=\qinv{ \epsilon md \alpha_I\beta_Jz_2}+\qinv{ \epsilon md \alpha_I\beta_JD_1z_2}\]
and applying $\Tr_{L/k}$ we get $0\in \operatorname{W}(k)$ since $y\not\in k$.
\end{enumerate}


\textbf{$P$ has at least one odd vertex}: we can assume that be $I+J$ is odd by Lemma \ref{lm: symmetry}. Then $\Tr_{E/k}\qinv{ \epsilon \alpha_I\beta_Jz_\circ^{I+J-e_1-e_2}}=\Tr_{E/k}\qinv{ \epsilon \alpha_I\beta_J}$ is equal to

\begin{center}
    \begin{tabular}{| l | l | l | l |}
    \hline
    \multirow{2}{*}{$d$ odd} & $\frac{m}{d}$ odd & \multicolumn{2}{|c|}{$\qinv{ \epsilon \alpha_I\beta_J}$} \\
    \cline{2-4}
     & $\frac{m}{d}$ even& \multicolumn{2}{|c|}{ $\qinv{ \epsilon\alpha_I\beta_J}+\qinv{ \epsilon \alpha_I\beta_JD_1}$}  \\ \hline
    \multirow{4}{*}{$d$ even} &\multirow{2}{*}{ $\frac{m}{d}$ odd} & $\Delta i_2\cdot r+\Delta j_2\cdot s$ odd& $\qinv{ \epsilon\alpha_I\beta_J}$+$\qinv{ \epsilon\alpha_I\beta_JD_2'D_1}$ \\ \cline{3-4} & & $\Delta i_2\cdot r+\Delta j_2\cdot s$ even & $\qinv{ \epsilon\alpha_I\beta_J}$+$\qinv{ \epsilon\alpha_I\beta_JD_2'}$\\
    \cline{2-4}
      &\multirow{2}{*}{ $\frac{m}{d}$ even} & $\Delta i_2\cdot r+\Delta j_2\cdot s$ odd& $\qinv{ \epsilon\alpha_I\beta_J}$+$\qinv{ \epsilon\alpha_I\beta_JD_1}$ \\ \cline{3-4} & &$\Delta i_2\cdot r+\Delta j_2\cdot s$ even & $\qinv{ \epsilon\alpha_I\beta_J}$+$\qinv{ \epsilon\alpha_I\beta_JD_1}$+$\qinv{ \epsilon\alpha_I\beta_JD_2'}$+$\qinv{ \epsilon\alpha_I\beta_JD_2'D_1}$\\
      \hline
    \end{tabular}
\end{center}
in $\operatorname{W}(k)$ by Proposition \ref{prop:traces} and \eqref{eq:D1}, \eqref{eq:D2} and \eqref{eq:D2'}.\medskip

By Lemma \ref{lm:m odd}, our statement follows if \textbf{$m$ is odd}: For $m$ odd, both $d$ and $\frac{m}{d}$ must be odd. Thus we get 
\[\widetilde{\operatorname{mult}}_p(C_1,C_2)=\qinv{ \epsilon \alpha_I\beta_J}+\frac{m-1}{2}\;h\in \GW(k)\]
where $I$ and $J$ are the unique choice such that $I+J=(1,1)$ in $\Z/2\Z\times \Z/2\Z$.\medskip

\textbf{Assume $d$ is odd and $\frac{m}{d}$ is even}:
Since we assume $d=\gcd(\Delta  i_1,\Delta j_1)$ to be odd, at least one out of $\Delta i_1$ and $\Delta j_1$ must be odd. Furthermore, we know that $\Delta i_1\cdot \Delta j_2\equiv \Delta i_2\cdot \Delta j_2\mod 2$ by \eqref{eq:m}. There are three possible cases.
\begin{enumerate}
    \item $\Delta i_1\equiv \Delta j_2\equiv \Delta i_2\equiv \Delta j_1\equiv 1\mod 2$: Then $I+J$ and $I'+J'$ are odd and $I+J'$ and $I'+J$ are not. In this case, $\frac{\Delta i_1}{d}$ and $\frac{\Delta j_1}{d}$ are both odd, and thus 
    \[\qinv{ \epsilon\alpha_I\beta_J}+\qinv{\epsilon\alpha_I\beta_JD_1}=\qinv{ \epsilon\alpha_I\beta_J}+\qinv{\epsilon\alpha_{I'}\beta_{J'}}.\]
    \item $\Delta i_1\equiv 1\mod 2$ and $\Delta j_2\equiv\Delta j_1 \equiv 0\mod 2$: Then $I+J$ and $I+J'$ are odd while $I'+J$ and $I'+J'$ are not. Then $\frac{\Delta i_1}{d}$ is odd and $\frac{\Delta j_1}{d}$ is even and 
        \[\qinv{ \epsilon\alpha_I\beta_J}+\qinv{\epsilon\alpha_I\beta_JD_1}=\qinv{ \epsilon\alpha_I\beta_J}+\qinv{-\epsilon\alpha_{I}\beta_{J'}}.\]
    \item $\Delta j_1\equiv 1\mod 2$ and $\Delta i_1\equiv\Delta i_2 \equiv 0\mod 2$: Then $I+J$ and $I'+J$ are odd while $I+J'$ and $I'+J'$ are not. Then $\frac{\Delta i_1}{d}$ is even and $\frac{\Delta j_1}{d}$ is odd and 
        \[\qinv{ \epsilon\alpha_I\beta_J}+\qinv{\epsilon\alpha_I\beta_JD_1}=\qinv{ \epsilon\alpha_I\beta_J}+\qinv{-\epsilon\alpha_{I'}\beta_{J}}.\]
\end{enumerate}

\textbf{$d$ is even and $\frac{m}{d}$ is odd}: Since $d$ is even, both $\Delta i_1$ and $\Delta j_1$ are even and since 
$\frac{m}{d}$ equals $\vert \frac{\Delta i_1}{d}\cdot \Delta j_2-\frac{\Delta j_1}{d}\cdot \Delta i_2\vert$ and is odd, at least one out of $\Delta i_2$ and $\Delta j_2$ is odd.
\begin{enumerate}
    \item If $\Delta i_2\equiv\Delta j_2\equiv 1\mod 2$, then $I+J$ and $I'+J'$ are odd, but $I+J'$ and $I'+J$ are not. Then $\Delta i_2\cdot r+\Delta j_2\cdot s\equiv r+s\mod 2$.
      \begin{enumerate}[label*=\arabic*.]
    \item     If $r+s$ is odd, then either $r$ is odd and $s$ is even or the other way round. If $r$ is odd and $s$ is even, then $\frac{\Delta i_1}{d}$ must be odd because of \eqref{eq:ra+ba=1}. Furthermore, $\frac{\Delta j_1}{d}$ must be even, otherwise $\frac{m}{d}=\vert\frac{\Delta i_1}{d}\Delta j_2-\frac{\Delta j_1}{d}\Delta i_2\vert$ would be even. Thus, we get
    \[\qinv{ \epsilon \alpha_I\beta_J}+\qinv{\epsilon\alpha_I\beta_JD_2'D_1}=\qinv{ \epsilon \alpha_I\beta_J}+\qinv{\epsilon \alpha_{I'}\beta_{J'}}.  \]
    By the same argument, we get the same if $r$ is even and $s$ is odd.
    \item 
    If $r+s$ is even, then both  $r$ and $s$ must be odd since they cannot both be even because of \eqref{eq:ra+ba=1}. In this case we get
    \[\qinv{ \epsilon \alpha_I\beta_J}+\qinv{\epsilon\alpha_I\beta_JD_2'}=\qinv{ \epsilon \alpha_I\beta_J}+\qinv{\epsilon \alpha_{I'}\beta_{J'}}.  \]
  \end{enumerate}
    \item If $\Delta i_2$ is odd and $\Delta j_2$ is even, then $I+J$ and $I+J'$ are odd and $I'+J$ and $I'+J'$ are not. 
    \begin{enumerate}[label*=\arabic*.]
    \item If $r\cdot\Delta i_2+s\cdot\Delta j_2\equiv r\cdot\Delta i_2\equiv r\equiv 1\mod 2$, then also $\frac{\Delta j_1}{d}\equiv1 \mod 2$ since we have that $\frac{\Delta i_1}{d}\Delta j_2+\frac{\Delta j_1}{d}\Delta i_2\equiv \frac{m}{d}\equiv 1\mod 2$. Thus $r+\frac{\Delta j_1}{d}\equiv 0\mod 2$. Furthermore, in this case $s+\frac{\Delta i_1}{d}\equiv 1\mod 2$, since otherwise $\frac{\Delta i_1}{d}\cdot r+\frac{\Delta j_1}{d}\cdot s=1$ would be even. So we get in this case that
    \[\qinv{ \epsilon \alpha_I\beta_J}+\qinv{ \epsilon\alpha_I\beta_JD_1D_2'}=\qinv{ \epsilon \alpha_I\beta_J}+\qinv{ -\epsilon\alpha_I\beta_{J'}}. \]
    \item If $\Delta i_2\cdot r+\Delta j_2\cdot s\equiv 0\mod 2$ then $r$ must be even. Thus $s$ must be odd by \eqref{eq:ra+ba=1} and we get
    \[\qinv{ \epsilon \alpha_I\beta_J}+\qinv{ \epsilon\alpha_I\beta_JD_2'}=\qinv{ \epsilon \alpha_I\beta_J}+\qinv{ -\epsilon\alpha_I\beta_{J'}}. \]
  \end{enumerate}
  \item In case $\Delta i_2$ is even and $\Delta j_2$ is odd, we have that $I+J$ and $I'+J$ are odd, and $I+J'$ and $I'+J'$ are not and we get 
  \[\qinv{ \epsilon \alpha_I\beta_J}+\qinv{ -\epsilon\alpha_{I'}\beta_{J}} \]
  by the same argument as in the case above.\bigskip
  
\end{enumerate}

\textbf{$d$ even and $\frac{m}{d}$ even}:
\begin{enumerate}
    \item If $\Delta i_2\cdot r+\Delta j_2\cdot s$ is odd, then at least one out of $\Delta i_2$ and $\Delta j_2$ must be odd.
    \begin{enumerate}[label*=\arabic*.]
    \item $\Delta i_2\equiv\Delta j_2\equiv 1\mod 2$: Then $\frac{\Delta j_1}{d}\equiv \frac{\Delta i_1}{d}\equiv 1\mod 2$ since $\frac{m}{d}$ is even and $\frac{\Delta j_1}{d}$ and $\frac{\Delta i_1}{d}$ cannot both be even since they are coprime. In this case, $I+J$ and $I'+J'$ are odd and $I+J'$ and $I'+J$ are not. We get 
    \[\qinv{ \epsilon \alpha_I\beta_J}+\qinv{\epsilon \alpha_I\beta_JD_1}=\qinv{ \epsilon \alpha_I\beta_J}+\qinv{\epsilon \alpha_{I'}\beta_{J'}}.\]
    \item If $\Delta i_2$ is odd and $\Delta j_2$ is even, then $\frac{\Delta j_1}{d}$ is even, since $\frac{m}{d}$ is even. Then $\frac{\Delta i_1}{d}$ must be odd since $\gcd(\frac{\Delta i_1}{d},\frac{\Delta j_1}{d})=1$. So $I+J$ and $I+J'$ are even while $I'+J$ and $I'+J'$ are not. We get
    \[\qinv{ \epsilon \alpha_I\beta_J}+\qinv{\epsilon \alpha_I\beta_JD_1}=\qinv{ \epsilon \alpha_I\beta_J}+\qinv{-\epsilon \alpha_{I}\beta_{J'}}.\]
    \item If $\Delta i_2$ is even and $\Delta j_2$ is odd, we know that $\frac{\Delta i_1}{d}$ is even and thus $\frac{\Delta j_1}{d}$ is odd by the same argument as in the case above. We get that $I+J$ and $I'+J$ are odd while $I+J'$ and $I'+J'$ are not and 
    \[\qinv{ \epsilon \alpha_I\beta_J}+\qinv{\epsilon \alpha_I\beta_JD_1}=\qinv{ \epsilon \alpha_I\beta_J}+\qinv{-\epsilon \alpha_{I'}\beta_{J}}.\]
  \end{enumerate}
  \item If $\Delta i_2\cdot r+\Delta j_2\cdot s$ is even, then $\Delta i_2$ and $\Delta j_2$ must both be even:\\
  We know that $\frac{\Delta i_1}{d}\cdot r+\frac{\Delta j_1}{d}\cdot s= 1$ and $\frac{\Delta i_1}{d}\cdot \Delta j_2\equiv\frac{\Delta j_1}{d}\cdot \Delta i_2\mod 2$ and one gets a contradiction to $\Delta i_2\cdot r+\Delta j_2\cdot s$ being even if one assumes that $\Delta i_2$ or $\Delta j_2$ is odd.\\
  So we get
  \begin{align*}&\qinv{ \epsilon\alpha_I\beta_J} +
  \qinv{ \epsilon\alpha_I\beta_JD_1}+
  \qinv{ \epsilon\alpha_I\beta_JD_2'}+
  \qinv{ \epsilon\alpha_I\beta_JD_1D_2'}\\
  =&\qinv{ \epsilon\alpha_I\beta_J} +
  \qinv{ -\epsilon\alpha_{I'}\beta_J}+
  \qinv{- \epsilon\alpha_I\beta_{J'}}+
  \qinv{ \epsilon\alpha_{I'}\beta_{J'}}.\end{align*}
\end{enumerate}





\end{proof}



%\subsection{Enriched intersection multiplicity using the B\'{e}zoutian}
%Let $I=(i_1,i_2)$, $J=(j_1,j_2)$, $I'=(i_1',i_2')$ and $J'=(j_1',j_2')$ be tuples of non-negative integers. Set $\Delta I\coloneqq I'-I$ and $\Delta J\coloneqq J'-J$.
%Let
%\[f_1=\alpha_Ix_1^{i_1}x_2^{i_2}+\alpha_{I'}x_1^{i_1'}x_2^{i_2'}\]
%and 
%\[f_2=\beta_Jx_1^{j_1}x_2^{j_2}+\beta_{J'}x_1^{j_1'}x_2^{j_2'}.\]

%Let $\mathfrak{m}$ be the maximal ideal corresponding to $p$. {\color{red} explain what $p$, it should be the the initial of the tropical intersection point we want to compute the intersection multiplicity at.}

%We compute the local $\A^1$-degree of $(f_1,f_2):\A^2_k\longrightarrow \A^2_k$ at $p$ using the B\'{e}zoutian form \eqref{eq:Bezoutian}. 

%We have 
%\begin{align*}\Delta_{1,1}&=\frac{\alpha_IX_1^{i_1}X_2^{i_2}+\alpha_{I'}X_1^{i_1'}X_2^{i_2'}-\alpha_IY_1^{i_1}X_2^{i_2}-\alpha_{I'}Y_1^{i_1'}X_2^{i_2'}}{X_1-Y_1}\\
%%\end{align*}

%One computes that the determinant of $(\Delta_{i,j})$ where $\Delta_{i,j}$ is defined as in \eqref{eq:Delta} equals
%\begin{align}
%\begin{split}
%\label{eq:detDelta}
%    &\det (\Delta_{i,j})=\\
%    &\alpha_I\beta_J\left(\sum_{i=0}^{i_1-1}\sum_{j=0}^{j_2-1}X_1^iY_1^{i_1+j_1-1-i}X_2^{i_2+j_2-1-j}Y_2^j-\sum_{i=0}^{j_1-1}\sum_{j=0}^{i_2-1}X_1^iY_1^{i_1+j_1-1-i}X_2^{i_2+j_2-1-j}Y_2^j\right)\\
%    +&\alpha_{I'}\beta_J\left(\sum_{i=0}^{i_1'-1}\sum_{j=0}^{j_2-1}X_1^iY_1^{i_1'+j_1-1-i}X_2^{i_2'+j_2-1-j}Y_2^j-\sum_{i=0}^{j_1-1}\sum_{j=0}^{i_2'-1}X_1^iY_1^{i_1'+j_1-1-i}X_2^{i_2'+j_2-1-j}Y_2^j\right)\\
%    +&\alpha_I\beta_{J'}\left(\sum_{i=0}^{i_1-1}\sum_{j=0}^{j_2'-1}X_1^iY_1^{i_1+j_1'-1-i}X_2^{i_2+j_2'-1-j}Y_2^j-\sum_{i=0}^{j_1'-1}\sum_{j=0}^{i_2-1}X_1^iY_1^{i_1+j_1'-1-i}X_2^{i_2+j_2'-1-j}Y_2^j\right)\\
%    +&\alpha_{I'}\beta_{J'}\left(\sum_{i=0}^{i_1'-1}\sum_{j=0}^{j_2'-1}X_1^iY_1^{i_1'+j_1'-1-i}X_2^{i_2'+j_2'-1-j}Y_2^j-\sum_{i=0}^{j_1'-1}\sum_{j=0}^{i_2'-1}X_1^iY_1^{i_1'+j_1'-1-i}X_2^{i_2'+j_2'-1-j}Y_2^j\right).
%\end{split}
%\end{align}

%To compute the B\'{e}zoutian form we need to find a basis of $Q=\frac{k[x_1,x_2]_\mathfrak{m}}{(f_1,f_2)}$. Let $d\coloneqq\gcd(\Delta i_1,\Delta j_1)$ where $\Delta i_1=i_1'-i_1$ and $\Delta j_1=j_1'-j_1$.



%\begin{equation}
%\label{eq:alpha}
%    \alpha_Ix_1^{i_1}x_2^{i_2}+\alpha_{I'}x_1^{i_1'}x_2^{i_2'}=0 \Leftrightarrow -\frac{\alpha_{I}}{\alpha_{I'}}=x_1^{\Delta i_1}x_2^{\Delta i_2}
%\end{equation}
%and 
%\begin{equation}
%\label{eq:beta}
%beta_Jx_1^{j_1}x_2^{j_2}+\beta_{J'}x_1^{j_1'}x_2^{j_2'}=0\Leftrightarrow -\frac{\beta_{J}}{\beta_{J'}}=x_1^{\Delta j_1}x_2^{\Delta j_2}.
%\end{equation}


%Then $\eqref{eq:alpha}^{-\frac{\Delta j_1}{d}}\cdot \eqref{eq:beta}^{\frac{\Delta i_1}{d}}$ yields
%\begin{equation}
%\label{eq:x2}
%    x_2^{\pm\frac{m}{d}}=\left(-\frac{\alpha_{I'}}{\alpha_{I}}\right)^{\frac{\Delta j_1}{d}}\cdot \left(-\frac{\beta_{J}}{\beta_{J'}}\right)^{\frac{\Delta i_1}{d}}.
%\end{equation}

%Since $\operatorname{gcd}(\frac{\Delta i_1}{d},\frac{\Delta j_1}{d})=1$
%, there are $r,s\in \Z$ such that 
%\[
%    r\cdot \frac{\Delta i_1}{d}+s\cdot \frac{\Delta j_1}{d}=1.
%\]
%{\color{red} maybe we shouldn't call these $r$ and $s$}

%Now $\eqref{eq:alpha}^{r}\cdot \eqref{eq:beta}^s$ yields 
%\begin{equation}
%\label{eq:x1}
%    x_1^d=x_2^{-\Delta i_2\cdot r-\Delta j_2 \cdot s}\cdot \left(-\frac{\alpha_{I'}}{\alpha_I}\right)^r\cdot \left(-\frac{\beta_{J'}}{\beta_J}\right)^s.
%\end{equation}
%So we have the following basis for $Q$ 
%\begin{equation}
%\label{eq:basis}
%\{x_1^ay_1^b:a=0,\ldots,d-1,b=0,\ldots,\frac{m}{d}-1\}.\end{equation}

%We are interested in the image of $\det (\Delta_{i,j})$ in $\frac{k[X,Y]}{(f(X),f(Y))}$. The relations \eqref{eq:alpha} and \eqref{eq:beta} will kill of quite a lot of terms in \eqref{eq:detDelta}. We want to know what is left after the relations.

%Assume $X_1^iY_1^{A-i}X_2^{B-j}Y_2^j$ is not killed of by \eqref{eq:alpha} or \eqref{eq:beta} where $A$ is equals $i_1+j_1-1$, $i_1'+j_1-1$, $i_1+j_1'-1$ or $i_1'+j_1'-1$ and $B$ equals $i_2+j_2-1$, $i_2'+j_2-1$, $i_2+j_2'-1$ or $i_2'+j_2'-1$ respectively. The coefficient of $x_1^iy_1^{A-i}x_2^{B-j}y_2^j$ is $\alpha_I\beta_J$, $\alpha_{I'}\beta_{J}$, $\alpha_I\beta_{J'}$ or $\alpha_{I'}\beta_{J'}$ respectively. By \eqref{eq:x2} we know that $X_2^{2\frac{m}{d}}\in (k^{\times})^2$. Hence we can change the exponent of $X_2$ in the monomial $X_1^iY_1^{A-i}X_2^{B-j}Y_2^j$ by multiples of $2\frac{m}{d}$ and the coefficient of the monomial is only changed by a square in $k^{\times}$. By \eqref{eq:x2} we can replace $Y_1^{2d}$ by $Y_2^{2(-r\Delta i_2-s\Delta j_2)}$ and the coeffiecient of the resulting monomial only differs by a square from the coefficient we started with. Replacing $j$ by $j-(r\Delta i_2+s\Delta i_1)$ we get the following equivalence relation on the  monomials in \eqref{eq:detDelta}
%\[X_1^iY_1^{A-i}X_2^{B-j}Y_2^j \sim X_1^iY_1^{A+p\cdot 2d}X_2^{p\cdot 2(r\Delta i_2+s\Delta j_2)+q\cdot 2\frac{m}{d}}Y_2^j\]
%for $p,q\in \mathbb{Z}$.

%\begin{lm}
%For each $(i,j)\in \{0,\ldots,d-1\}\times\{0,\ldots,\frac{m}{d}-1\}$ there is exactly one basis element in \eqref{eq:basis} equivalent to  monomial in \eqref{eq:detDelta}.
%\end{lm}
%\begin{proof}
%Assume $x_1^iy_1^{a}x_2^by_2^j$ and $x_1^iy_1^{a'}x_2^{b'}y_2^j$ are both equivalent to a monomial in \eqref{eq:detDelta}. Then 
%\begin{align*}
 %   a&=A-i+p\cdot 2d\\
 %   b&=B-j+p\cdot2(r\Delta i_2+s\Delta j_2)+q\cdot 2\frac{m}{d}\\
 %   a'&=A'-i+p'\cdot 2d\\
 %   b'&=B'-j+p'\cdot2(r\Delta i_2+s\Delta j_2)+q'\cdot 2\frac{m}{d}
%\end{align*}
%for some $p,q,p',q'\in \Z$ {\color{red} explain what $A,B,A',B'$ are...}
 
%We have the following possibilities for $a-a'$
%\[a-a'=\begin{cases}
%0+(p'-p)\cdot 2d  \\
%\pm \Delta i_1+(p'-p)\cdot 2d\\
%\pm \Delta j_1+(p'-p)\cdot 2d\\
%\pm (\Delta i_1-\Delta j_1)+(p'-p)\cdot 2d\\
%\pm (\Delta i_1+\Delta j_1)+(p'-p)\cdot 2d.
%\end{cases}
%\]
%Since $a,a'\in \{0,\ldots,d-1\}$ we know that $\vert a-a'\vert\le d-1$. Furthermore, $d$ divides $\Delta i_1$ and $\Delta j_1$. 
%So the only possibility is that $a=a'$, and in particular $p=p'$.

%For $b-b'$ we have 
%\[b-b'=\begin{cases}
%0+(q'-q)\cdot 2\frac{m}{d}  \\
%\pm \Delta i_2+(q'-q)\cdot 2\frac{m}{d}\\
%\pm \Delta j_2+(q'-q)\cdot 2\frac{m}{d}\\
%\pm (\Delta i_2-\Delta j_2)+(q'-q)\cdot 2\frac{m}{d}\\
%\pm (\Delta i_2+\Delta j_2)+(q'-q)\cdot 2\frac{m}{d}.
%\end{cases}
%\]

%Since $\vert b-b'\vert\le \frac{m}{d}-1$. {\color{red} do case distinction... if $\Delta i_1$, $\Delta j_1$, $\Delta i_1+\Delta j_1$ resp $\Delta i_1-\Delta j_1$ equals $0$, in the corresponding case $\frac{m}{d}$ divides $\Delta i_2$, $\Delta j_2$, $\Delta i_2+\Delta j_2$ resp $\Delta i_2-\Delta j_2$...}
%we get $a=a'$ and $b=b'$.
%\end{proof}

%It follows that the image of $\det(\Delta_{i,j})$ in %$\frac{k[X,Y]}{(f(X),f(Y))}$ has at most $d\cdot \frac{m}{d}$ summands (one for each $(i,j)\in \{0,\ldots,d-1\}\times\{0,\ldots,\frac{m}{d}-1\}$). 
%When we call the elements in the basis \eqref{eq:basis} $a_1,\ldots,a_m$ and write the image of $\det(\Delta_{i,j})$ in $\frac{k[X,Y]}{(f(X),f(Y))}$ as
%\[\sum_{i,j=1}^mB_{i,j}a_i(X)a_j(Y)\]
%for some $B_{i,j}\in k$, we know by \eqref{eq:Bezoutian} that the matrix $(B_{i,j})$ of the local $\A^1$-degree of $f$ at $p$. In particular, $B_{i,j}$ has full rank. Hence, the image of $\det(\Delta_{i,j})$ in $\frac{k[X,Y]}{(f(X),f(Y))}$ has exactly $m$ summands. The formula works in any characteristic, so the coefficients of theses summands must be
%$\pm \alpha_I\beta_J$, $\pm \alpha_{I'}\beta_J$,$\pm \alpha_I\beta_{J'}$ or $\pm \alpha_{I'}\beta_{J'}$.


%{\color{red} continue}






